At the same age, metallicity, and alpha-enhancement, sodium is a more effective tracer of the young and old sequences of the Milky Way disc

Trends in the enrichment of elements with stellar ages are a powerful avenue to identify unexplained origins of the elements. We investigate the stellar abundance trends of low to intermediate-mass stars using the GALAH DR3 high-resolution spectroscopic dataset of 6234 solar-type stars. Our study explores the elemental abundance [X/Fe] of sodium (Na) with age. We find a pronounced enrichment in [Na/Fe] at super solar metallicity (i.e., [Fe/H] above 0) in the old sequence of Milky Way disc stars, a trend demanding a deeper understanding of the underlying source(s) responsible for the nucleosynthesis. This progressive [Na/Fe] enrichment at the young end of the old sequence has essential implications for Galactic archaeology. In this work, we propose a novel selection technique for separating the Milky Way's thick and thin disc stellar populations (i.e., old and young sequences) based on the observed [Na/Fe] rise of roughly 0.1 dex for stars around 5 - 8 Gyr old. We also compare our selection method to the conventional [Mg/Fe] vs [Fe/H] selection approach, and we find that our new Na-based selection method better disentangles the overlap between young- and old-sequence disc stars at these intermediate ages. This is especially true at super solar [Fe/H], where [Mg/Fe] vs [Fe/H] or [alpha/Fe] vs [Fe/H] separation approaches exhibit a lot of overlap. This new selection method should help us better understand the Milky Way disc's formation history.

==> text/slope_5.0_6.5_Al.tex <==
$0.0263 \pm 0.0041\,\mathrm{dex/Gyr}$


==> text/slope_5.0_6.5_Ba.tex <==
$-0.0652 \pm 0.0052\,\mathrm{dex/Gyr}$


==> text/slope_5.0_6.5_C.tex <==
$-0.0199 \pm 0.0078\,\mathrm{dex/Gyr}$


==> text/slope_5.0_6.5_Ca.tex <==
$-0.0059 \pm 0.0046\,\mathrm{dex/Gyr}$


==> text/slope_5.0_6.5_Co.tex <==
$-0.0698 \pm 0.0099\,\mathrm{dex/Gyr}$


==> text/slope_5.0_6.5_Cr.tex <==
$0.0388 \pm 0.0043\,\mathrm{dex/Gyr}$


==> text/slope_5.0_6.5_Cu.tex <==
$0.0723 \pm 0.0034\,\mathrm{dex/Gyr}$


==> text/slope_5.0_6.5_K.tex <==
$0.0021 \pm 0.0053\,\mathrm{dex/Gyr}$


==> text/slope_5.0_6.5_Mg.tex <==
$0.0119 \pm 0.0041\,\mathrm{dex/Gyr}$


==> text/slope_5.0_6.5_Mn.tex <==
$0.0516 \pm 0.0041\,\mathrm{dex/Gyr}$


==> text/slope_5.0_6.5_Ni.tex <==
$0.0433 \pm 0.0043\,\mathrm{dex/Gyr}$


==> text/slope_5.0_6.5_O.tex <==
$-0.0652 \pm 0.0084\,\mathrm{dex/Gyr}$


==> text/slope_5.0_6.5_Sc.tex <==
$0.0256 \pm 0.0031\,\mathrm{dex/Gyr}$


==> text/slope_5.0_6.5_Ti.tex <==
$-0.0144 \pm 0.0035\,\mathrm{dex/Gyr}$


==> text/slope_5.0_6.5_Ti2.tex <==
$0.0065 \pm 0.0037\,\mathrm{dex/Gyr}$


==> text/slope_5.0_6.5_V.tex <==
$0.0292 \pm 0.0094\,\mathrm{dex/Gyr}$


==> text/slope_5.0_6.5_Y.tex <==
$-0.0262 \pm 0.0071\,\mathrm{dex/Gyr}$


==> text/slope_5.0_6.5_Zn.tex <==
$0.0257 \pm 0.0051\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_Al.tex <==
$0.0066 \pm 0.0012\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_Ba.tex <==
$-0.0226 \pm 0.0016\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_C.tex <==
$-0.0145 \pm 0.0024\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_Ca.tex <==
$-0.0043 \pm 0.0014\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_Co.tex <==
$-0.0230 \pm 0.0031\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_Cr.tex <==
$0.0164 \pm 0.0013\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_Cu.tex <==
$0.0285 \pm 0.0010\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_K.tex <==
$-0.0051 \pm 0.0016\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_Mg.tex <==
$-0.0022 \pm 0.0012\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_Mn.tex <==
$0.0236 \pm 0.0012\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_Ni.tex <==
$0.0199 \pm 0.0013\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_O.tex <==
$-0.0339 \pm 0.0025\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_Sc.tex <==
$0.0062 \pm 0.0009\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_Ti.tex <==
$-0.0095 \pm 0.0011\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_Ti2.tex <==
$-0.0011 \pm 0.0012\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_V.tex <==
$0.0063 \pm 0.0027\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_Y.tex <==
$0.0027 \pm 0.0022\,\mathrm{dex/Gyr}$


==> text/slope_5.0_8.0_Zn.tex <==
$0.0092 \pm 0.0015\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_Al.tex <==
$-0.0113 \pm 0.0027\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_Ba.tex <==
$-0.0016 \pm 0.0035\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_C.tex <==
$-0.0125 \pm 0.0053\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_Ca.tex <==
$-0.0017 \pm 0.0031\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_Co.tex <==
$0.0544 \pm 0.0077\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_Cr.tex <==
$0.0092 \pm 0.0029\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_Cu.tex <==
$0.0080 \pm 0.0023\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_K.tex <==
$-0.0058 \pm 0.0035\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_Mg.tex <==
$-0.0090 \pm 0.0027\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_Mn.tex <==
$0.0137 \pm 0.0027\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_Ni.tex <==
$0.0064 \pm 0.0029\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_O.tex <==
$-0.0210 \pm 0.0056\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_Sc.tex <==
$-0.0052 \pm 0.0021\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_Ti.tex <==
$-0.0103 \pm 0.0024\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_Ti2.tex <==
$-0.0054 \pm 0.0029\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_V.tex <==
$-0.0019 \pm 0.0062\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_Y.tex <==
$0.0160 \pm 0.0048\,\mathrm{dex/Gyr}$


==> text/slope_6.5_8.0_Zn.tex <==
$-0.0076 \pm 0.0034\,\mathrm{dex/Gyr}$


==> text/table2.tex <==
\begin{tabular}{ccccccc}
        \hline \hline
        Element & Percentile & 3 & 5 & 7 & 9 \\
        \hline
        C & 16 &-0.128&-0.103&-0.080&-0.026\\
        C & 50 & -0.035 & -0.021 & 0.014 & 0.074\\
        C & 84 & 0.024 & 0.067 & 0.103 & 0.176\\
        O & 16 & -0.175 &-0.133&-0.081 &0.004 \\ 
        O & 50 &-0.116 &-0.051  &0.013 &0.098\\
        O & 84 &-0.050&0.047 & 0.106& 0.95\\ 
        Na & 16 & 0.126 & 0.015 &-0.003 &-0.031\\
        Na & 50 &0.159&0.068 &0.044& 0.023\ \\
        Na & 84  &0.212 &0.130&0.090&0.073\\
        Mg & 16  &-0.045&-0.053\ &-0.044 \ &-0.023\\
        Mg & 50  &0.002 \ &-0.060 \ &0.001 \ &0.031\\
        Mg & 84  &0.038 \ &0.037 \  &0.048&0.103\\
        Al & 16  &0.045 \ &0.001 \ &-0.001 \ &0.010\\
        Al & 50  &0.089 \ &0.056  \ &0.054 &0.068\\
        Al & 84 &0.120\ &0.106 \ &0.110 \  &0.166\\
        Si & 16 &-0.017 \ &-0.025 \ &-0.025 \ &-0.013\\
        Si & 50 &0.009 \ &0.004 \ &0.009 \ &0.027 \\
        Si & 84 &0.037 \ &0.032 \ & 0.042\  &0.069\\
        K & 16  &-0.075 \ &-0.072 \ &-0.069 \ &-0.055\\
        K & 50  &-0.008 \ &-0.015 \ &-0.003 \ &0.021 \ \\
        K & 84  &0.010 \ &0.064 \ &0.089 \ &0.122\\
        Ca & 16   &-0.045 \ &-0.066 \ &-0.057 \ &-0.045\\
        Ca & 50   &0.000 \ &-0.007 \ &0.002 \ &0.016\\
        Ca & 84   &0.041 \ &0.048 \ &0.058 \  &0.077\\
        Sc & 16  &0.052 \ &0.016 \ &0.017 \ &0.017\\
        Sc & 50  &0.092 \ &0.058 \ &0.056 \ &0.064\\
        Sc & 84  &0.117 \ &0.096\ &0.095 \  &0.113\\
        Ti & 16  &-0.035 \ &-0.038 \ &-0.028 \ &-0.015\\
        Ti & 50  & 0.005\ &0.004 \ &0.018 \ &0.041\\
        Ti & 84  &0.033 \ &0.049 \ &0.070 \  &0.103\\
        Ti2& 16  &-0.055\ &-0.057 \ &-0.053 \ &-0.034\\
        Ti2 & 50  &-0.009 \ &0.001 \ &0.008 \ &0.029 \\
        Ti2 & 84  &0.036 \ &0.062 \ &0.073 \  &0.093\\
        V & 16 &-0.083 \ &-0.138 \ &-0.145 \ &-0.16\\
        V & 50 &0.003 &\-0.026 \ &-0.046&-0.041\\
        V& 84 &0.053 \ &0.075 \ &0.080 \  &0.093\\
        Cr & 16   &-0.046 \ &-0.097 \ &-0.114 \ &-0.120\\
        Cr & 50  &0.009 \ &-0.040 \ &-0.062 \ &-0.076\\
        Cr & 84   &0.057 \ &0.030 \ &0.006 \ &-0.011 \\
        Mn & 16   &0.046\ &-0.022 \ &-0.051 \ &-0.080\\
        Mn & 50  &0.081 \ &0.032 \ &0.000 \ &-0.036\\
        Mn & 84  &0.130 \ &0.084 \ &0.051 \ &0.012 \\
        Co& 16  &-0.103 \ &-0.105 \ &-0.098 \ &-0.072\\
        Co & 50 &-0.009 \ &0.024 \ &0.044 \ &0.104\\
        Co & 84 \ &0.146 \ &0.255 \ &0.359 \ &0.460\\
        Ni & 16  &0.016 \ &-0.059 \ &-0.086 \ &-0.105\\
        Ni & 50  &0.069\ &0.004 \ &-0.022 \ &-0.046\\
        Ni & 84   &0.097\ &0.065 \ &0.032 \  &0.010\\
        Cu & 16   &0.105 \ & -0.006\ &-0.032 \ &-0.046\\
        Cu & 50   &0.157 \ &0.077 \ &0.045 \ &0.017\\
        Cu & 84   &0.205 \ &0.149 \ &0.106 \ &0.087\\
        Zn & 16   &0.037 \ &-0.025 \ &-0.034 \ &-0.019\\
        Zn & 50   &0.070 \ &0.037 \ &0.032 \ &0.048\\
        Zn & 84   &0.114 \ &0.100 \ &0.094 \  &0.117\\
        Y & 16   &-0.153 \ &-0.179 \ &-0.216 \ &-0.253\\
        Y & 50   &-0.092 \ &-0.103 \ &-0.126 \ &-0.169 \\
        Y & 84  &-0.037 \ &-0.022 \ &-0.030 \  &-0.066\\
        Ba & 16  &-0.220 \ &-0.178 \ &-0.148 \ &-0.158\\
        Ba & 50  &-0.151 \ &-0.093 \ &-0.072 \ &-0.082\\
        Ba & 84  &-0.076 \ &-0.002 \ &0.007 \  &0.00\\
        La & 16  &0.109 \ &0.164 \ &0.187 \ &0.217\\
        La & 50  &0.205 \ &0.269 \ &0.309 \ &0.334\\
        La & 84 &0.375 \ &0.406 \ &0.464 \ &0.534\\
        \hline \hline
    \end{tabular}

==> text/tabular_bin_slopes.tex <==
\begin{tabular}{ccccccc}
\hline \hline
Atomic Number & Element & Gradient $5.0-8.0\,\,\mathrm{Gyr}$  & Gradient $6.5-8.0\,\,\mathrm{Gyr}$ & Gradient $5.0-6.5\,\mathrm{Gyr}$ \\%& $\Delta$Fit \\
& & $\mathrm{dex\,Gyr^{-1}}$ & $\mathrm{dex\,Gyr^{-1}}$ & $\mathrm{dex\,Gyr^{-1}}$\\
\hline
6 & C & $\,\,\,\,-0.0145 \pm 0.0024$ & $\,\,\,\,-0.0125 \pm 0.0053$ & $\,\,\,\,-0.0199 \pm 0.0078$ \\
8 & O & $\,\,\,\,-0.0339 \pm 0.0025$ & $\,\,\,\,-0.0210 \pm 0.0056$ & $\,\,\,\,-0.0652 \pm 0.0084$ \\
11 & Na & $0.0260 \pm 0.0009$ & $0.0066 \pm 0.0021$ & $0.0673 \pm 0.0031$ \\
12 & Mg & $\,\,\,\,-0.0022 \pm 0.0012$ & $\,\,\,\,-0.0090 \pm 0.0027$ & $0.0119 \pm 0.0041$ \\
13 & Al & $0.0066 \pm 0.0012$ & $\,\,\,\,-0.0113 \pm 0.0027$ & $0.0263 \pm 0.0041$ \\
14 & Si & $\,\,\,\,-0.0011 \pm 0.0011$ & $\,\,\,\,-0.0068 \pm 0.0024$ & $0.0053 \pm 0.0035$ \\
19 & K & $\,\,\,\,-0.0051 \pm 0.0016$ & $\,\,\,\,-0.0058 \pm 0.0035$ & $0.0021 \pm 0.0053$ \\
20 & Ca & $\,\,\,\,-0.0043 \pm 0.0014$ & $\,\,\,\,-0.0017 \pm 0.0031$ & $\,\,\,\,-0.0059 \pm 0.0046$ \\
21 & Sc & $0.0062 \pm 0.0009$ & $\,\,\,\,-0.0052 \pm 0.0021$ & $0.0256 \pm 0.0031$ \\
22 & Ti & $\,\,\,\,-0.0095 \pm 0.0011$ & $\,\,\,\,-0.0103 \pm 0.0024$ & $\,\,\,\,-0.0144 \pm 0.0035$ \\
22 & Ti2 & $\,\,\,\,-0.0011 \pm 0.0012$ & $\,\,\,\,-0.0054 \pm 0.0029$ & $0.0065 \pm 0.0037$ \\
24 & V & $0.0063 \pm 0.0027$ & $\,\,\,\,-0.0019 \pm 0.0062$ & $0.0292 \pm 0.0094$ \\
25 & Cr & $0.0164 \pm 0.0013$ & $0.0092 \pm 0.0029$ & $0.0388 \pm 0.0043$ \\
27 & Mn & $0.0236 \pm 0.0012$ & $0.0137 \pm 0.0027$ & $0.0516 \pm 0.0041$ \\
28 & Co & $\,\,\,\,-0.0230 \pm 0.0031$ & $0.0544 \pm 0.0077$ & $\,\,\,\,-0.0698 \pm 0.0099$ \\
29 & Ni & $0.0199 \pm 0.0013$ & $0.0064 \pm 0.0029$ & $0.0433 \pm 0.0043$ \\
30 & Cu & $0.0285 \pm 0.0010$ & $0.0080 \pm 0.0023$ & $0.0723 \pm 0.0034$ \\
39 & Zn & $0.0092 \pm 0.0015$ & $\,\,\,\,-0.0076 \pm 0.0034$ & $0.0257 \pm 0.0051$ \\
56 & Y & $0.0027 \pm 0.0022$ & $0.0160 \pm 0.0048$ & $\,\,\,\,-0.0262 \pm 0.0071$ \\
57 & Ba & $\,\,\,\,-0.0226 \pm 0.0016$ & $\,\,\,\,-0.0016 \pm 0.0035$ & $\,\,\,\,-0.0652 \pm 0.0052$ \\
\hline \hline
\end{tabular}


==> text/tabular_slopes.tex <==
\begin{tabular}{ccccccc}
\hline \hline
Atomic Number & Element & Gradient $5.0-8.0\,\,\mathrm{Gyr}$  & Gradient $6.5-8.0\,\,\mathrm{Gyr}$ & Gradient $5.0-6.5\,\mathrm{Gyr}$ \\%& $\Delta$Fit \\
& & $\mathrm{dex\,Gyr^{-1}}$ & $\mathrm{dex\,Gyr^{-1}}$ & $\mathrm{dex\,Gyr^{-1}}$\\
\hline
6 & C & $-0.0145 \pm 0.0024$ & $-0.0125 \pm 0.0053$ & $-0.0199 \pm 0.0078$ \\
8 & O & $-0.0339 \pm 0.0025$ & $-0.0210 \pm 0.0056$ & $-0.0652 \pm 0.0084$ \\
11 & Na & $\,\,\,\,0.0260 \pm 0.0009$ & $\,\,\,\,0.0066 \pm 0.0021$ & $\,\,\,\,0.0673 \pm 0.0031$ \\
12 & Mg & $-0.0022 \pm 0.0012$ & $-0.0090 \pm 0.0027$ & $\,\,\,\,0.0119 \pm 0.0041$ \\
13 & Al & $\,\,\,\,0.0066 \pm 0.0012$ & $-0.0113 \pm 0.0027$ & $\,\,\,\,0.0263 \pm 0.0041$ \\
14 & Si & $-0.0011 \pm 0.0011$ & $-0.0068 \pm 0.0024$ & $\,\,\,\,0.0053 \pm 0.0035$ \\
19 & K & $-0.0051 \pm 0.0016$ & $-0.0058 \pm 0.0035$ & $\,\,\,\,0.0021 \pm 0.0053$ \\
20 & Ca & $-0.0043 \pm 0.0014$ & $-0.0017 \pm 0.0031$ & $-0.0059 \pm 0.0046$ \\
21 & Sc & $\,\,\,\,0.0062 \pm 0.0009$ & $-0.0052 \pm 0.0021$ & $\,\,\,\,0.0256 \pm 0.0031$ \\
22 & Ti & $-0.0095 \pm 0.0011$ & $-0.0103 \pm 0.0024$ & $-0.0144 \pm 0.0035$ \\
22 & Ti2 & $-0.0011 \pm 0.0012$ & $-0.0054 \pm 0.0029$ & $\,\,\,\,0.0065 \pm 0.0037$ \\
24 & V & $\,\,\,\,0.0063 \pm 0.0027$ & $-0.0019 \pm 0.0062$ & $\,\,\,\,0.0292 \pm 0.0094$ \\
25 & Cr & $\,\,\,\,0.0164 \pm 0.0013$ & $\,\,\,\,0.0092 \pm 0.0029$ & $\,\,\,\,0.0388 \pm 0.0043$ \\
27 & Mn & $\,\,\,\,0.0236 \pm 0.0012$ & $\,\,\,\,0.0137 \pm 0.0027$ & $\,\,\,\,0.0516 \pm 0.0041$ \\
28 & Co & $-0.0230 \pm 0.0031$ & $\,\,\,\,0.0544 \pm 0.0077$ & $-0.0698 \pm 0.0099$ \\
29 & Ni & $\,\,\,\,0.0199 \pm 0.0013$ & $\,\,\,\,0.0064 \pm 0.0029$ & $\,\,\,\,0.0433 \pm 0.0043$ \\
30 & Cu & $\,\,\,\,0.0285 \pm 0.0010$ & $\,\,\,\,0.0080 \pm 0.0023$ & $\,\,\,\,0.0723 \pm 0.0034$ \\
39 & Zn & $\,\,\,\,0.0092 \pm 0.0015$ & $-0.0076 \pm 0.0034$ & $\,\,\,\,0.0257 \pm 0.0051$ \\
56 & Y & $\,\,\,\,0.0027 \pm 0.0022$ & $\,\,\,\,0.0160 \pm 0.0048$ & $-0.0262 \pm 0.0071$ \\
57 & Ba & $-0.0226 \pm 0.0016$ & $-0.0016 \pm 0.0035$ & $-0.0652 \pm 0.0052$ \\
\hline \hline
\end{tabular}

